A 13-Billion-Year View of Galaxy Growth: Metallicity Gradient Evolution from the Local Universe to $z=9$ with JWST and Archival Surveys

The galaxy gas-phase metallicity gradients have been extensively studied over the past four decades, both in the local and high-redshift universe, as they trace the baryon cycle and growth of galaxies. With the unprecedented spatial resolution and sensitivity of JWST, it is now possible to measure metallicity and its radial gradients out to redshifts as high as $z = 9$. Here, we present a sample of 455 spectroscopically confirmed galaxies from redshifts $1.7 \lesssim z \lesssim 9$ that are spatially resolved on sub-kiloparsec (kpc) scales by deep JWST NIRCam or NIRISS Wide Field Slitless Spectroscopy (WFSS). Synthesizing these new JWST observations with legacy observations from the literature, we observe that at redshift $z > 5$, galaxy centers are more metal-rich, exhibiting negative metallicity gradients of $\sim-0.4$ dex kpc$^{-1}$. These gradients flatten over time, reaching near-zero around $z \approx 2$, coinciding with the peak of the cosmic star formation rate. Beyond this point, the gradients become negative again at lower redshifts approaching $z=0$. This evolution likely reflects transitions in galaxy formation modes: an inside-out growth phase dominated by intense central star formation with inefficient feedback and limited gas mixing during ``cosmic dawn", enhanced gas mixing due to feedback-driven wind and gas accretion at ``cosmic noon", and a later phase of slow evolution and reduced feedback toward the present day. These physical processes, including gas accretion and feedback, not only regulate star and galaxy formation on a cosmic scale but also shape the evolutionary pathways of individual galaxies over cosmic time.

==> preamble.tex <==
%%<<140818>> update this preamble file in terms of the beamer version
%%<<141022>> merged the beamer version and the manu version together and re-locate it at latex_refs/

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% page setup
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%---------------- Margin setup with header and footer, see https://en.wikibooks.org/wiki/LaTeX/Page_Layout
%%\setlength{\paperheight}{29.7cm}  \setlength{\paperwidth}{21cm}       % A4paper size
%\setlength{\paperheight}{11in}  \setlength{\paperwidth}{8.5in}         % letter size
%\setlength{\textheight}{9.5in}  \setlength{\textwidth}{7in}
%\setlength{\oddsidemargin}{-0.25in}  \setlength{\evensidemargin}{-0.25in}
%\setlength{\headheight}{0in}
%\setlength{\headsep}{.3in}
%\setlength{\footskip}{.35in}
%\setlength{\tabcolsep}{0in}
%\setlength{\topmargin}{-0.3in}
%\setlength{\topskip}{0in}
%\setlength{\voffset}{-0.1in}
%---------------- alternative way of setting the margins
%\usepackage{geometry}
%\newcommand{\marg}{1in}
%\geometry{letterpaper,tmargin=\marg,bmargin=\marg,lmargin=\marg,rmargin=\marg,headheight=0in,headsep=.27in,footskip=.4in}
%-------------- sets \parskip to be a flexible "glue" length with natural length 1ex and can shrink to 1ex-0.4ex and stretch to
%               1ex+0.4ex to pad out a page to the required height.
%\setlength{\parskip}{0.4ex plus 0.2ex minus 0.2ex}
%\setlength{\parindent}{0in}        % 首行缩进
% \flushbottom                % makes all text pages the same height

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% packages and settings useful globally
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{longtable}
\usepackage[english]{babel} % default (American) English hyphenation
\usepackage[utf8]{inputenc} % useful to type directly diacritic characters
\usepackage[T1]{fontenc}    % Use vector fonts, so it zooms properly in on-screen viewing software
\usepackage{mathtools, cuted}
\DeclareUnicodeCharacter{0301}{/}
\DeclareUnicodeCharacter{2212}{-}
\usepackage{ae,aecompl}
%\usefont{T1}{tnr}{m}{sl}    % conflicting txfonts!
%\usepackage{fancyhdr}       % fancy header
\usepackage{pgf,pgfarrows,pgfnodes,pgfautomata,pgfheaps}
\usepackage{graphicx}       % you can specify [driver] (e.g. [pdftex]) which is the dvi to postscript program
%\usepackage{natbib}         % enables the use of \citep and others; see http://merkel.zoneo.net/Latex/natbib.php
\usepackage{url}            % enables the use of url web links
\usepackage{grffile}        % enables dots and underscores in .pdf filenames
\usepackage{mathtools}      % enables the use of various environments work, e.g., |align|, |dcases|, define symbols (see below), etc.
% \usepackage{bbold}          % enables the use of \mathbb{1} as the identity matrix
% \newcommand{\bb}{\mathbb}
% \usepackage{bbm}            % enables the use of bold Greek symbols
% \newcommand{\bs}{\boldsymbol}
\DeclareGraphicsRule{.tif}{.png}{.jpg}{.bmp}
\usepackage{multirow}       % enables the use of \multirow{num}{*}{text} in deluxetable
\usepackage{xspace}         % enables the use of \xspace in defining macros
%\usepackage{epstopdf}
% \usepackage{ccaption}       % continuation of caption for figures containing multiple floats
%\usepackage{booktabs}       % enable \toprule, etc. in tables in proposals
% \usepackage{wrapfig}

%-------------- spacing, see: https://tex.stackexchange.com/questions/196967/double-or-one-half-spacing
%\usepackage{setspace}
%\doublespacing
%\frenchspacing

\usepackage{tikz,lipsum,lmodern}
\usepackage[most]{tcolorbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% disable for the use of jwst proposal template
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amsmath,amssymb,amsxtra,amsfonts}   % to use pmatrix, etc.
\usepackage{txfonts}
\newcommand{\kms}{\ensuremath{\rm km~s^{-1}}\xspace}
\newcommand{\lya}{\textrm{Ly}\ensuremath{\alpha}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% special packages and corresponding usages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-------------- provide circled numbers
%\usepackage{tikz}
%\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=2pt] (char) {#1};}}
%-------------- use \mathsmaller and \mathlarger to resize math symbols
%\usepackage{relsize}
%-------------- for dynamic display of tables, see
%               http://www.math-linux.com/latex-26/article/how-to-make-a-presentation-with-latex-introduction-to-beamer
%\usepackage{colortbl}
%-------------- correct total number of pages for appendix, have to be commented off when using \appendix in ms.tex, and for poster
%               http://texblog.org/2012/05/24/correct-total-number-of-pages-with-backup-slides-in-beamer-presentations/
%\usepackage{appendixnumberbeamer}
%-------------- strikethrough in beamer itemize, see
%               http://tex.stackexchange.com/questions/35767/in-beamer-how-to-strike-through-an-item-after-displaying
%\usepackage{ulem}       % turn \emph to \underline
%\renewcommand<>{\sout}[1]{\alt#2{\beameroriginal{\sout}{#1}}{#1}}
%-------------- set up {itemize, enumerate} from scratch!. will mess up \\tableofcontents. Should leave it commented!
%				http://tex.stackexchange.com/questions/24371/does-enumitem-conflict-with-beamer-for-lists
%\usepackage{enumitem}
%\setitemize{label=\usebeamerfont*{itemize item}%
%  \usebeamercolor[fg]{itemize item}
%  \usebeamertemplate{itemize item}}
%-------------- create checkbox and todolist in itemize (the latter needs to enable enumitem), see
%               http://tex.stackexchange.com/questions/247681/how-to-create-checkbox-todo-list
%\newlist{todolist}{itemize}{2}
%\setlist[todolist]{label=$\square$}    % NOTE: you can use \begin{itemize} with \item[$\square$] to replace todolist
%\usepackage{pifont}
%\newcommand{\cmark}{\ding{51}}%
%\newcommand{\done}{\rlap{$\square$}{\raisebox{2pt}{\large\hspace{1pt}\cmark}}\hspace{-2.5pt}}
%\newcommand{\xmark}{\ding{55}}%
%\newcommand{\wontfix}{\rlap{$\square$}{\large\hspace{1pt}\xmark}}
%-------------- include videos, works for .flv, .mov format
%\usepackage{media9}
%-------------- encourage a break at this point
%\newcommand{\smallspace}{\vspace{3cm}\goodbreak}
%\newcommand{\bigspace}{\vspace{4.5cm}\goodbreak}
%\newcommand{\biggerspace}{\vspace{5.5cm}\goodbreak}
%-------------- put the points in the left margin, see latex_manuscripts/reference/hw3_sol_fin.tex
%\reversemarginpar
%\newcommand{\worth}[1]
%        {\mbox{}\marginpar{\em #1}\nolinebreak}%puts value in margin
%-------------- Flexible typesetting of table and figure floats, see: https://ctan.org/pkg/ctable
%\usepackage{ctable}
%-------------- add texts in box, see: https://tex.stackexchange.com/questions/36524/how-to-put-a-framed-box-around-text-math-environment/36528
%\usepackage{tcolorbox}
%-------------- define new column type, see: https://tex.stackexchange.com/questions/257128/how-does-the-newcolumntype-command-work
%\usepackage{array}
%\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{5pt}}m{#1}}


% -----------------------------------------------------------------------------------------------
% Turning references and citations into hyperlinks in color
\usepackage{color}         % using color package; put color boxes around text: \fcolorbox{frame colour}{background colour}{text}
\definecolor{gold}{rgb}{1,0.80,0}
\definecolor{orange}{rgb}{1,0.5,0}
\definecolor{midgray}{gray}{0.3}
\definecolor{lblue}{rgb}{0,0.2,0.6}
\definecolor{dgreen}{rgb}{0.1,0.6,0.3}
\definecolor{purple}{rgb}{0.5019607843137255,0.0,0.5019607843137255}

% -----------------------------------------------------------------------------------------------
% Reference a section by ``section XX'', without generating text like ``subsection XX'' as is done by \autoref.
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\Eqref}[1]{Equation~(\ref{#1})}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% only necessary for beamer, aastex63
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{deluxetable}
% - - - - - - - - have to comment off when using beamer
%\usepackage[colorlinks=true,citecolor=lblue,linkcolor=dgreen]{hyperref}    % does not work for draft, beamer, aastex63
%\urlstyle{rm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% only necessary for poster
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{wrapfig}
%\usepackage{caption}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% only necessary for emulateapj
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% - - - - - - - - already defined
\newcommand\farcs{\mbox{$.\!^{\prime\prime}$}}    % arcsec with a decimal point in front
\newcommand\farcm{\mbox{$.\mkern-4mu^\prime$}}      % arcmin with a decimal point in front
\newcommand{\arcsec}{\mbox{$^{\prime\prime}$}\xspace}  % the unit of arcsec, NOTE: can try adding "\!" before "^" to shorten space
\newcommand{\arcmin}{\mbox{$\!^{\prime}$}\xspace}          % the unit of arcmin
\newcommand{\arcdeg}{\mbox{$^{\circ}$}\xspace}             % the unit of arcdeg
% - - - - - - - - have to comment off when using emulateapj
\usepackage{marvosym}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% mathematical symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\font\fb=''[cmr10]'' %for use with \LaTeX command
% pre-existing symbols: \exp, \ln, \log
%\newcommand{\rmd}{\textrm{d}}
%\def\d{\textrm{d}}   % NOTE: \newcommad doesn't work but this works!
\def\prt{\partial}
\def\cP{{\cal P}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\non}{\nonumber}
\newcommand{\ba}{\begin{align}}
\newcommand{\ea}{\end{align}}
\newcommand{\nt}{\notag}
\def\abs#1{\left|{#1}\right|}
\newcommand{\avg}[1]{\left<#1\right>}
%-------- provide define symbols
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}
%-------- formatted arrows
\newcommand{\Ra}{\ensuremath{\Rightarrow}\xspace}
\newcommand{\ra}{\ensuremath{\rightarrow}\xpace}
\newcommand{\lra}{\ensuremath{\Leftrightarrow}\xspace}
% Statistical mean (angle brackets)
\newcommand{\stmean}[1]{\langle{#1}\rangle}
\newcommand{\logg}{\log_{10}}	% base-10 logarithm
% Spatial-curvature function in cosmological distances.
\DeclareMathOperator{\sk}{S}
% Trace of a linear operator or matrix
\DeclareMathOperator{\tr}{tr}
% Differential (must be upright Roman letter, per MNRAS)
\DeclareMathOperator{\ud}{d}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% (astro)physical units and quantities
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% - - - - - - - - quantities
\newcommand{\Msun}{\ensuremath{M_\odot}\xspace}
\newcommand{\Rsun}{\ensuremath{R_\odot}\xspace}
\newcommand{\Lsun}{\ensuremath{L_\odot}\xspace}
\newcommand{\thE}{\ensuremath{\theta_{\rm E}}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\zspec}{\ensuremath{z_{\rm spec}}\xspace}
\newcommand{\zphot}{\ensuremath{z_{\rm phot}}\xspace}
\newcommand{\Mstar}{\ensuremath{M_\ast}\xspace}
\newcommand{\Lstar}{\ensuremath{L_\ast}\xspace}
\newcommand{\Sstar}{\ensuremath{\Sigma_\ast}\xspace}
\newcommand{\oh}{\ensuremath{12+\log({\rm O/H})}\xspace}
\newcommand{\Av}{\ensuremath{A_{\rm V}}\xspace}
\newcommand{\Rv}{\ensuremath{R_{\rm V}}\xspace}
\newcommand{\Te}{\ensuremath{T_{\rm e}}\xspace}
\def\ne{\ensuremath{n_{\rm e}}\xspace}
\newcommand{\SFR}{\ensuremath{{\rm SFR}}\xspace}
\newcommand{\Mgas}{\ensuremath{M_{\rm gas}}\xspace}
\newcommand{\Sgas}{\ensuremath{\Sigma_{\rm gas}}\xspace}
\newcommand{\fgas}{\ensuremath{f_{\rm gas}}\xspace}
\newcommand{\Zgas}{\ensuremath{Z_{\rm gas}}\xspace}
\newcommand{\tage}{\ensuremath{t_{\rm age}}\xspace}
\newcommand{\Vrot}{\ensuremath{V_{\rm rot}}\xspace}
\newcommand{\reff}{\ensuremath{r_{\rm eff}}\xspace}
\newcommand{\Dn}{\ensuremath{{\rm D}_n(4000)}\xspace}
\newcommand{\HdA}{\ensuremath{{\rm H}\delta_A}\xspace}
\newcommand{\scrit}{\ensuremath{\sigma_{\rm crit}}\xspace}
\newcommand{\fesc}{\ensuremath{f_{\rm esc}}\xspace}
\newcommand{\xion}{\ensuremath{\xi_{\rm ion}}\xspace}
\newcommand{\tauIGM}{\ensuremath{\tau_{\rm IGM}}\xspace}
\newcommand{\Muv}{\ensuremath{M_{\rm UV}}\xspace}

% - - - - - - - - units
\newcommand{\eV}{\ensuremath{\rm eV}\xspace}
\newcommand{\pc}{\ensuremath{\rm pc}\xspace}
\newcommand{\kpc}{\ensuremath{\rm kpc}\xspace}
\newcommand{\Mpc}{\ensuremath{\rm Mpc}\xspace}
\newcommand{\K}{\ensuremath{\rm K}\xspace}
\newcommand{\mK}{\ensuremath{\rm mK}\xspace}
\newcommand{\Hunit}{\ensuremath{\rm km~s^{-1}~Mpc^{-1}}\xspace}
\newcommand{\Funit}{\ensuremath{\rm erg~s^{-1}~cm^{-2}}\xspace}
\newcommand{\Flam}{\ensuremath{\rm erg~s^{-1}~cm^{-2}~\AA^{-1}}\xspace}
\newcommand{\Fnu}{\ensuremath{\rm erg~s^{-1}~cm^{-2}~Hz^{-1}}\xspace}
\newcommand{\muJy}{\ensuremath{\mu\rm Jy}\xspace}
\newcommand{\SBunit}{\ensuremath{\rm erg~s^{-1}~cm^{-2}~arcsec^{-2}}\xspace}
\newcommand{\magarcs}{\ensuremath{\rm mag~arcsec^{-2}}\xspace}
\newcommand{\Msunyr}{\ensuremath{\Msun~\mathrm{yr}^{-1}}\xspace}
\newcommand{\yr}{\ensuremath{\rm yr}\xspace}
\newcommand{\Myr}{\ensuremath{\rm Myr}\xspace}
\newcommand{\Gyr}{\ensuremath{\rm Gyr}\xspace}
\def\micron{\ensuremath{\mu\textrm{m}}\xspace}  % better than the default \micron, which does not use \xspace
% - - - - - - - - copied from Tucker
%\newcommand{\rhosfr}{\dot{\rho}_{\star}}
%\newcommand{\rhouv}{\rho_{\mathrm{UV}}}
%\newcommand{\rhosfrunit}{\mathrm{M}_{\sun}~\mathrm{yr}^{-1}~\mathrm{Mpc}^{-3}}
%\newcommand{\rhouvunit}{\mathrm{ergs}~\mathrm{s}^{-1}~\mathrm{Hz}^{-1}\mathrm{Mpc}^{-3}}
%\newcommand{\luvunit}{\mathrm{ergs}~\mathrm{s}^{-1}~\mathrm{Hz}^{-1}}
%\newcommand{\funit}{\mathrm{ergs}~\mathrm{s}^{-1}~\mathrm{cm}^{-2}}
% - - - - - - - - copied from Louis, but not yet tried
%\newcommand\arcmin{\mbox{$^\prime$}}%
%\newcommand\arcsec{\mbox{$^{\prime\prime}$}}%
%\newcommand\fd{\mbox{$.\!\!^{\textrm d}$}}%
%\newcommand\fh{\mbox{$.\!\!^{\textrm h}$}}%
%\newcommand\fm{\mbox{$.\!\!^{\textrm m}$}}%
%\newcommand\fs{\mbox{$.\!\!^{\textrm s}$}}%
%\newcommand\fdg{\mbox{$.\!\!^\circ$}}%
%\newcommand\fp{\mbox{$.\!\!^{\scriptscriptstyle\textrm p}$}}%
%\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
%\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% astrophysical aliases and jargons
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\ionp[2]{#1$\;${\scshape{#2}}}      % ion permitted transitions, i.e., C IV = \ionp{C}{iv}
\newcommand\ionf[2]{[#1$\;${\scshape{#2}}]}    % ion forbidden transitions, i.e., [O III] = \ionf{O}{iii}
\newcommand\ions[2]{#1$\;${\scshape{#2}}]}     % ion semi-forbidden transitions, i.e., C III] = \ions{C}{iii}
\newcommand{\Ha}{\textrm{H}\ensuremath{\alpha}\xspace}
\newcommand{\Hb}{\textrm{H}\ensuremath{\beta}\xspace}
\newcommand{\Hg}{\textrm{H}\ensuremath{\gamma}\xspace}
\newcommand{\Hd}{\textrm{H}\ensuremath{\delta}\xspace}
\newcommand{\HII}{\textrm{H}\textsc{ii}\xspace}
\newcommand{\HI}{\textrm{H}\textsc{i}\xspace}
\newcommand{\Htwo}{\textrm{H}\ensuremath{_2}\xspace}
\newcommand{\He}{\textrm{He}\xspace}
\newcommand{\OI}{[\textrm{O}~\textsc{i}]\xspace}
\newcommand{\OII}{[\textrm{O}~\textsc{ii}]\xspace}
\newcommand{\OIII}{[\textrm{O}~\textsc{iii}]\xspace}
\newcommand{\CIII}{\textrm{C}~\textsc{iii}]\xspace}
\newcommand{\NII}{[\textrm{N}~\textsc{ii}]\xspace}
\newcommand{\SII}{[\textrm{S}~\textsc{ii}]\xspace}
\newcommand{\NeIII}{[\textrm{Ne}~\textsc{iii}]\xspace}
\newcommand{\HeII}{\textrm{He}~\textsc{ii}\xspace}
\newcommand{\CIV}{\textrm{C}~\textsc{iv}\xspace}
\newcommand{\SiIV}{\textrm{Si}~\textsc{iv}\xspace}
\newcommand{\CII}{\textrm{C}~\textsc{ii}\xspace}


\newcommand{\sersic}{S\'{e}rsic\xspace}
% - - - - - - - - astrometric filters
\def\U{\ensuremath{U_{360}}\xspace}     % only for LBT U-band imaging
\def\B{\ensuremath{B_{435}}\xspace}
\def\V{\ensuremath{V_{606}}\xspace}
\def\I{\ensuremath{I_{814}}\xspace}
\def\Y{\ensuremath{Y_{105}}\xspace}
\def\J{\ensuremath{J_{125}}\xspace}
\def\JH{\ensuremath{JH_{140}}\xspace}
\def\H{\ensuremath{H_{160}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% my specific macros for objects, software, instruments, telescopes, projects
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% - - - - - - - - celestial objects
\newcommand{\clyi}{MACS1149.6+2223\xspace}
\newcommand{\cler}{Abell 2744\xspace}
\newcommand{\clsan}{Abell 370\xspace}
\newcommand{\clsi}{MACS0416.1-2403\xspace}
\newcommand{\clwu}{MACS0717.5+3745\xspace}
\newcommand{\clliu}{RXJ2248.7-4431\xspace}
\newcommand{\clqi}{RXJ1347.5-1145\xspace}
\newcommand{\clba}{MACS0744.9+3927\xspace}
\newcommand{\cljiu}{MACS2129.4-0741\xspace}
\newcommand{\clshi}{MACS1423.8+2404\xspace}

% - - - - - - - - software
\newcommand{\pylf}{\textsc{pyLensFix}\xspace}
\newcommand{\lf}{\textsc{LensFix}\xspace}
\newcommand{\sw}{\textsc{SWunited}\xspace}
\newcommand{\sex}{\textsc{SExtractor}\xspace}
\newcommand{\emc}{\textsc{Emcee}\xspace}
\newcommand{\linmix}{\textsc{linmix}\xspace}
\newcommand{\adriz}{\textsc{AstroDrizzle}\xspace}
\newcommand{\dpac}{\textsc{DrizzlePac}\xspace}
\newcommand{\fast}{\textsc{FAST}\xspace}
\newcommand{\galfit}{\textsc{Galfit}\xspace}
\newcommand{\axe}{\textsc{aXe}\xspace}
\def\lt{\textsc{Lenstool}\xspace}
\newcommand{\glafic}{\textsc{Glafic}\xspace}
\newcommand{\gasoline}{\textsc{Gasoline}\xspace}
\newcommand{\ramses}{\textsc{Ramses}\xspace}
\newcommand{\SJ}{\textsc{Sharon \& Johnson}\xspace}
\newcommand{\grzl}{\textsc{Grizli}\xspace}
\newcommand{\burst}{\textsc{Starburst99}\xspace}
\newcommand{\tphot}{\textsc{T-PHOT}\xspace}
\newcommand{\bagp}{\textsc{BAGPIPES}\xspace}
\newcommand{\phut}{\textsc{Photutils}\xspace}
\newcommand{\msa}{\textsc{msaexp}\xspace}
\newcommand{\ppxf}{\textsc{pPXF}\xspace}


% - - - - - - - - projects, telescopes, instruments
\newcommand{\jwst}{\textit{JWST}\xspace}
\newcommand{\planck}{\textit{Planck}\xspace}
\newcommand{\hst}{\textit{HST}\xspace}
\newcommand{\hubble}{\textit{Hubble}\xspace}
\newcommand{\spitzer}{\textit{Spitzer}\xspace}
\newcommand{\herschel}{\textit{Herschel}\xspace}
\newcommand{\chandra}{\textit{Chandra}\xspace}
\newcommand{\glass}{\textit{GLASS}\xspace}
\newcommand{\clear}{\textit{CLEAR}\xspace}
\newcommand{\wisp}{\textit{WISP}\xspace}
\newcommand{\clash}{\textit{CLASH}\xspace}
\newcommand{\candels}{\textit{CANDELS}\xspace}
\newcommand{\uvc}{\textit{UVCANDELS}\xspace}
\newcommand{\hff}{\textit{HFF}\xspace}
\newcommand{\muse}{\textit{MUSE}\xspace}
\newcommand{\kmos}{\textit{KMOS}\xspace}
\newcommand{\keck}{\textit{Keck}\xspace}
\newcommand{\deimos}{\textit{DEIMOS}\xspace}
\newcommand{\mosfire}{\textit{MOSFIRE}\xspace}
\newcommand{\surfsup}{\textit{SURFSUP}\xspace}
\newcommand{\kd}{\textit{KMOS}$^{3\rm D}$\xspace}
\newcommand{\sdss}{\textit{SDSS}\xspace}
\def\clash{\textit{CLASH}\xspace}
\def\mosdef{\textit{MOSDEF}\xspace}
\newcommand{\vlt}{\textit{VLT}\xspace}
\newcommand{\osiris}{\textit{OSIRIS}\xspace}
\newcommand{\sinf}{\textit{SINFONI}\xspace}
\newcommand{\ngrst}{\textit{NGRST}\xspace}
\newcommand{\niriss}{\textit{NIRISS}\xspace}
\newcommand{\mmth}{\textit{MAMMOTH}\xspace}
\newcommand{\mg}{\textit{MAMMOTH-Grism}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% format, wording and abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\etal{et al.\xspace}
\def\ie{i.e.\xspace}
\def\eg{e.g.\xspace}
\def\etc{etc.\xspace}
\def\aka{a.k.a.\xspace}
\def\vsv{vis-\'a-vis\xspace}
\renewcommand\({\left(}
\renewcommand\){\right)}
%\renewcommand\[{\left[}
%\renewcommand\]{\right]}

% - - - - - - - - word combo
% \newcommand\mm{metallicity map\xspace}
% \newcommand\mms{metallicity maps\xspace}
% \newcommand\mg{metallicity gradient\xspace}
% \newcommand\mgs{metallicity gradients\xspace}
% \newcommand\Mgs{Metallicity gradients\xspace}
% \newcommand\mgm{metallicity gradient measurement\xspace}
% \newcommand\mgms{metallicity gradient measurements\xspace}
% \newcommand\sr{spatially resolved\xspace}
% \newcommand\srs{spatially resolved spectroscopy\xspace}
% \newcommand\sra{spatially resolved analysis\xspace}
% \newcommand\gp {gas-phase\xspace}
% \newcommand\gpm{gas-phase metallicity\xspace}
% \newcommand\subr{surface brightness\xspace}        % <<160715>> NOTE: cannot re-DEF \sb
\newcommand\sfr{star-formation rate\xspace}
\newcommand\sfh{star-formation history\xspace}
\newcommand\sfms{star-formation main sequence\xspace}

% - - - - - - - - specially formated words
\newcommand{\el}[1]{\ensuremath{\textrm{EL}_{#1}}}
\newcommand{\obs}{\textrm{o}}
\newcommand{\theo}{\textrm{t}}
\newcommand{\ext}{\textrm{ext}}
\def\det{\textrm{det}}
\newcommand\refe{\textrm{ref}}
\newcommand\pa{\textrm{PA}}

\def\p{{\rm prior}}
\def\fid{{\rm fid}}
\def\lnk{\kappa}
\def\lnkp{\kappa'}
%\newcommand{\n}{\noindent}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% lensing quantities and parameters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\xa}{\alpha}
\newcommand{\xb}{\beta}
\newcommand{\xk}{\kappa}
\newcommand{\xg}{\gamma}
%\newcommand{\xg}[1]{|\gamma #1|}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% cosmological parameters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Or} {\ensuremath{\Omega_{\rm{r}}}\xspace}
\newcommand{\Om} {\ensuremath{\Omega_{\rm{m}}}\xspace}
\newcommand{\Ok} {\ensuremath{\Omega_{\rm{k}}}\xspace}
\newcommand{\Ol} {\ensuremath{\Omega_{\Lambda}}\xspace}
\newcommand{\Obh}{\ensuremath{\Omega_{\rm{b}}h^2}\xspace}
\newcommand{\Ob} {\ensuremath{\Omega_{\rm{b}}}\xspace}
\newcommand{\Onu}{\ensuremath{\Omega_\nu}\xspace}
\newcommand{\fnu}{\ensuremath{f_{\nu}}\xspace}
\newcommand{\Och}{\ensuremath{\Omega_{\rm{DM}}h^2}\xspace}
\newcommand{\Oc} {\ensuremath{\Omega_{\rm{DM}}}\xspace}
\newcommand{\ns} {\ensuremath{n_{\rm s}}\xspace}
\newcommand{\As} {\ensuremath{A_{\rm s}}\xspace}
%\newcommand{\nt} {\ensuremath{n_{\rm t}}\xspace}
%\newcommand{\At} {\ensuremath{A_{\rm t}}\xspace}
\newcommand{\thA}{\ensuremath{\theta_{\rm A}}\xspace}
%\newcommand{\run}{\ensuremath{{dn_s \over d\ln k}}\xspace}
\newcommand{\neff}{\ensuremath{N_\textrm{eff}}\xspace}
\newcommand{\mnu}{\ensuremath{\sum{m_{\nu}}}\xspace}
\newcommand{\yhe}{\ensuremath{Y_p}\xspace}
%\newcommand{\nrun}{\ensuremath{dn_s/d\ln k}\xspace}
\newcommand{\Map}[1]{\left<M^2_\textrm{ap}\right>( #1 )}
\newcommand{\map}{\ensuremath{\left<M^2_\textrm{ap}\right>}\xspace}
\newcommand{\chiH}{\ensuremath{\chi_\textrm{H}}\xspace}
\newcommand{\n}{\ensuremath{{\nu}\rm}\xspace}
\newcommand{\nue}{\ensuremath{{\nu}_{\rm e}}\xspace}
\newcommand{\num}{\ensuremath{{\nu}_{\rm \mu}}\xspace}
\newcommand{\nut}{\ensuremath{{\nu}_{\rm \tau}}\xspace}
\newcommand{\da}{\ensuremath{D_{\rm A}}\xspace}
\newcommand{\dl}{\ensuremath{D_{\rm L}}\xspace}
%\newcommand{\pripk}{\ensuremath{P_{\textrm{pri}}(k)}}
\newcommand{\taueq}{\ensuremath{\tau_{\rm eq}}\xspace}

%%------------------------------------- begin of a slide ----------------------------------------
%\begin{frame}{}
%    block options: alertblock, exampleblock
%
%\end{frame}
%%===================================== end of a slide ==========================================

%%------------------------------------- begin of a slide ----------------------------------------
%\begin{frame}{}
%    \vspace*{-.3em}
%    \begin{columns}[c]
%        \begin{column}{5.5cm}
%        \end{column}
%        \hspace*{-3em}
%        \begin{column}{5.5cm}
%        \end{column}
%    \end{columns}
%\end{frame}
%%===================================== end of a slide ==========================================

%= = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =
% fancy header setup in P88
%\documentclass{book}
%\usepackage{fancyhdr}
%\pagestyle{fancy}
%% with this we ensure that the chapter and section
%% headings are in lowercase.
%\renewcommand{\chaptermark}[1]{%
%        \markboth{#1}{}}
%\renewcommand{\sectionmark}[1]{%
%        \markright{\thesection\ #1}}
%\fancyhf{}  % delete current header and footer
%\fancyhead[LE,RO]{\bfseries\thepage}
%\fancyhead[LO]{\bfseries\rightmark}
%\fancyhead[RE]{\bfseries\leftmark}
%\renewcommand{\headrulewidth}{0.5pt}
%\renewcommand{\footrulewidth}{0pt}
%\addtolength{\headheight}{0.5pt} % space for the rule
%\fancypagestyle{plain}{%
%   \fancyhead{} % get rid of headers on plain pages
%   \renewcommand{\headrulewidth}{0pt} % and the line
%}

%= = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =
%%% Figures
%\begin{figure}
%    \centering
%    \includegraphics[width=0.8\textwidth]{}
%    \caption[]{
%    \label{fig:XXX}}
%\end{figure}
%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -


%= = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =
% self-learning notes
%= = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =
%<<160301>>
%   \textrm does not work with \ensuremath, use \mathrm instead! but \mathrm{} cannot only contain one symbol
%<<190409>>
%   dropping \centering saves space!
%<<191223>>
%   put \vspace*{-1.1em} inside \begin{center} \end{center} makes it more consistent!




